Continual Pre-training of Language Models

Language models (LMs) have been instrumental for the rapid advance of natural language processing. This paper studies continual pre-training of LMs, in particular, continual domain-adaptive pre-training (or continual DAP-training). Existing research has shown that further pre-training an LM using a domain corpus to adapt the LM to the domain can improve the end-task performance in the domain. This paper proposes a novel method to continually DAP-train an LM with a sequence of unlabeled domain corpora to adapt the LM to these domains to improve their end-task performances. The key novelty of our method is a soft-masking mechanism that directly controls the update to the LM. A novel proxy is also proposed to preserve the general knowledge in the original LM. Additionally, it contrasts the representations of the previously learned domain knowledge (including the general knowledge in the pre-trained LM) and the knowledge from the current full network to achieve knowledge integration. The method not only overcomes catastrophic forgetting, but also achieves knowledge transfer to improve end-task performances. Empirical evaluation demonstrates the effectiveness of the proposed method.

==> deprecated/sections/abstract.tex <==
\begin{abstract}
{\color{red}Language models (LMs) have been instrumental for the recent rapid advance of natural language processing. Existing research has shown that post-training or adapting a LM using an unlabeled topical/domain corpus can improve the end-task performance in the domain.~This paper proposes a novel method to \textit{continually post-train} a LM with a sequence of unlabeled domain corpora to adapt the LM to these domains to improve their end-task performances.
{The key novelty of our method is a soft-masking mechanism that directly updates the LM by exploiting the over-parameterization property of LMs. A novel proxy is also proposed to preserve the general knowledge in the origianl LM. Additionally, it contrasts the previously learned domain representations and current domain representation to achieve a complementary effect.} As a result, the method not only overcomes \textit{catastrophic forgetting}, but also achieve \textit{knowledge transfer} across domains to improve the end-task performance compared to post-training each domain separately. Empirical evaluation demonstrates the effectiveness of the proposed method. \footnote{The code has been uploaded as supplementary materials.} }
 % The key innovation of our method is that it directly updates the MLM by exploiting the over-parameterization property of MLMs and by carefully detecting and soft-masking important and unimportant parameters in the MLM for continual training. This method not only overcomes catastrophic forgetting but also achieves knowledge transfer.
 % It computes the importance of attention heads and neurons % \zixuan{How about "importance of parameters (converted from importance of attention heads and neurons)" and then we simply used "importance of parameters" else where. Now we have many version of description of "importance of X"}
% for previous domains and soft-masks them based on the importance scores to deal with catastrophic forgetting and to encourage knowledge transfer. 
%Unlike many existing CL methods, our method needs no replay memory and no network expansion. Domain identification information is also not needed for end-task learning.



\end{abstract}

==> deprecated/sections/conclusion.tex <==

\section{Conclusion}
% \zixuan{conclusion not done, need to mention limiatation}
This paper studied task incremental learning (TIL) within the pre-trained RoBERTa to achieve both CF prevention and knowledge transfer.
It proposed a novel technique called ICB to leverage the RoBERTa for CL. The key idea of ICB is the importance controlled propagation in Transformer. The importance is computed to preserve both previous knowledge and pre-trained general knowledge so that effective knowledge transfer can be achieved. CF is prevented by a small adapter and a focus-shifting strategy. Experimental results showed that ICB markedly improves the performance of both the new task and the old tasks via knowledge transfer and is also effective at overcoming CF. 

\textit{Limitation}: The adapter 
% \zixuan{which one is better?}
can condition the Transformer for each task to help deal with CF, but it causes inefficiency. %The efficiency due to the use of adapter. Adapter can effectively condition the Transformer while adding new parameters to each layer of Transformer.
How to remove the need of such an additional module is left to our future work.

% (2) the needed hyper-parameter tuning for each datasets. A critical hyper-parameter is the temperature which control when to shift from adapter training to Transformer training. If it shifts too early, forgetting may occur; if too late, knowledge transfer may be too little.


==> deprecated/sections/experiments.tex <==

\section{Experiments}
\label{sec:experiments}

We follow the experiment setup in \cite{DBLP:journals/corr/abs-1909-08383} and use 
RoBERTa \cite{DBLP:journals/corr/abs-1907-11692}\footnote{\url{https://huggingface.co/roberta-base}} as the LM. In CL, after a domain is trained, its training data is no longer accessible. After all domains are incrementally learned, the final model is evaluated using fine-tuning end-tasks in all domains.
% In each experiment, we first continual DAP-training the LM and then fine-tuning it on the end-task. The final evaluation is based on the end-task results.



% We give the detail below.
% We first initialize the language model RoBERTa \cite{DBLP:journals/corr/abs-1907-11692} (our LM) with its corresponding pre-trained weights,\footnote{\url{https://huggingface.co/roberta-base}} and then further pre-train it with different approaches (see Table~\ref{tab:DAP-training_result}) using different unlabeled domain data (see Table~\ref{tab:dataset}) before fine-tuning on the end-tasks. The final evaluation are based on the end-task results.% We give the detail below.

\subsection{Datasets and Baselines}
\label{sec.data-baselines}


\textbf{Datasets:} 
Table \ref{tab:dataset} shows the statistics of the \textit{unlabeled domain corpora} for DAP-training and their corresponding \textit{end-task classification datasets}. We use 6 \textit{unlabeled domain datasets}:\footnote{We down-sampled the \textit{PubMed} due to its huge original size. In general, our datasets are much smaller comparing to previous work \cite{DBLP:conf/acl/GururanganMSLBD20} (which used more than 11GB of data for each domain). Our experiments showed that a smaller dataset is sufficient and more data does not help. It also requires much less computation resources.} 3 of them are about reviews: \textit{Yelp Restaurant} \cite{DBLP:conf/naacl/XuLSY19}, %\textit{Amazon Laptop} \cite{DBLP:conf/naacl/XuLSY19},
\textit{Amazon Phone} \cite{DBLP:conf/emnlp/NiLM19}, \textit{Amazon Camera} \cite{DBLP:conf/emnlp/NiLM19}; 3 of them are academic papers: \textit{ACL Papers} \cite{DBLP:conf/acl/LoWNKW20}, \textit{AI Papers} \cite{DBLP:conf/acl/LoWNKW20}, and \textit{PubMed Papers}\footnote{\url{https://pubmed.ncbi.nlm.nih.gov/}}.
% \zixuan{Within these 8 unsupervised datasets, we ... Need to mention what special things we have done and why} 
The corresponding \textit{end-task classification datasets} of these datasets are:\footnote{Our results are different from those presented in Table 5 of \cite{DBLP:conf/acl/GururanganMSLBD20} because we observe very high variances due to very small test sets and thus enlarge the test set and reduce the training set slightly.} \textit{Restaurant}\footnote{\url{https://alt.qcri.org/semeval2014/task4/}}, % \footnote{To be consistent with existing research \cite{tang-etal-2016-aspect}, examples with conflict polarities (both positive and negative sentiments are expressed about an aspect term) are not used.} 
% \cite{DBLP:conf/naacl/XuLSY19}
\textit{Phone} \cite{ding2008holistic,hu2004mining}, \textit{Camera} \cite{ding2008holistic,hu2004mining}\footnote{We use those domains related to ``Phone'' and ``Camera'' from the datasets in the two references.},
% Note that \cite{ding2008holistic} and \cite{hu2004mining} contain 9 and 5 domains, respectively. We extract those domains related to  from them.}, 
\textit{ACL} (ACL-ARC in \cite{DBLP:journals/tacl/JurgensKHMJ18}), \textit{AI} (SCIERC in \cite{DBLP:conf/emnlp/LuanHOH18}), and PubMed (CHEMPORT in \cite{kringelum2016chemprot}).  
% \bing{correct?} \zixuan{Now PubMed domain and task are of the same name. Do we want to change the domain name to "PubMed Papers"?}
% why we don't want to use their original name?} \bing{It will be confusing in the results tables}


\vspace{+1.5mm}
\noindent
\textbf{Baselines.} We use 15 baselines, including Non-continual learning (Non-CL) and continual learning (CL) baselines. All CL baselines  except DEMIX are not for learning unsupervised data. We adapt them and replace their backbone with RoBERTa. Details of each baseline is given in Appendix~\ref{ap:baseline}. % They cover non-DAP-training (RoBERTa), existing DAP-training (MLM), with RoBERTTa fixed (MLM(ADAP-traininger), MLM(Promnpt), KD, and AdaptedDeiT) and systems using contrastive learning (SimnCSE and TaCL).  

\textbf{Non-CL Baselines}: Each baseline here builds a separate model for each
task independently. 
\textbf{(1) RoBERTa}~\cite{DBLP:journals/corr/abs-1907-11692} uses the original RoBERTa for the end-task fine-tuning without DAP-training. \textbf{(2) RoBERTaDAP} uses the existing DAP-training method in~\cite{DBLP:conf/acl/GururanganMSLBD20}; \textbf{(3) AdapterDAP} adds adapter layers in Transformer for DAP-training~\cite{madotto2020continual,Houlsby2019Parameter}. Only the added adapters are trainable. In end-task fine-tuning, both RoBERTa and the adapters are trainable;  \textbf{(4) PromptDAP} is based on %adds a sequence of real vector tokens (called virtual tokens or prompt tokens) to the end of the original sequence
\cite{DBLP:conf/emnlp/LesterAC21}. In DAP-training, RoBERTa (the LM) is fixed and only the prompt tokens are trained. In end-task fine-tuning, both the LM and the trained prompt are trainable. % (CDS needs none of these).


\textbf{CL Baselines}: We use 2 naive baselines, which keep learning more domains/tasks with no mechanism dealing with forgetting or transfer. \textbf{(5) NCL} (Naive CL) continually DAP-trains the RoBERTa; and \textbf{(6) AdapterCL} (Continual learning with adapter)~\cite{Houlsby2019Parameter} continually DAP-trains the same set of adapters. % Both have no mechanism to deal with forgetting or transfer.

8 baselines are state-of-the-art CL systems: \textbf{(7) DEMIX (AdapterDEMIX)}~\cite{gururangan2021demix} adds a new adapter for each new domain and initializes it with the parameters of the previous adapter nearest to the new domain data; \textbf{(8) AdapterHAT}~\cite{ke2021adapting} uses HAT~\cite{Serra2018overcoming} within adapters. % with almost no forgetting. AdapterHAT adapts HAT to RoBERTa by applying it to the adapter layer (thus AdapterHAT); 
\textbf{(9) AdapterBCL}~\cite{ke2021adapting} is based on capsule networks. 
% to encourage transfer and the other one is similar to AdapterHAT to avoid forgetting; 
\textbf{(10) AdapterCLASSIC}~\cite{ke2021Classic} is based on contrastive learning. \textbf{(11) KD} is based on knowledge distillation % from the last DAP-trained LM to the current LM
~\cite{hinton2015distilling}. %\zixuan{now KD is very closed to (13), we probably want to say "based on knowledge distillation from last DAP-trained LM to the current LM"} % that computes the KL divergence distillation loss. % between the representations (the output before the masked language model prediction head) of each token of the previous DA-trained LM and current LM; 
\textbf{(12) EWC}~\cite{buzzega2020dark} is a popular
regularization-based method. \textbf{(13) DER++}~\cite{buzzega2020dark} is a replay method based on knowledge distillation. 16.4K tokens are saved for each domain in the replay memory, which is the largest memory we can use for the system to run. %\zixuan{we didn't give detail for all other baselines, why only give detail (16.4L...) for DER++ here? (why not in supplementary)}
\textbf{(14) HAT}~\cite{Serra2018overcoming} is a state-of-the-art \textit{parameter-isolation} method. HAT is applied to Transformer layers (including self-attention, intermediate and output layers). No adapters are used like AdapterHAT. {\color{black}\textbf{(15) HAT*} is a HAT variant using the same DAP-training, but all features \textit{from the LM} are used to do end-tasks (instead of only features from its domain sub-network as in HAT).} % \zixuan{added HAT*}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=\textwidth]{results.png}
% \end{figure*}

\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|ccccccccccccccc}
\specialrule{.2em}{.1em}{.1em}
\multirow{2}{*}{Category} & Domain & \multicolumn{2}{c}{Restaurant} & \multicolumn{2}{c}{ACL} & \multicolumn{2}{c}{AI} & \multicolumn{2}{c}{Phone} & PubMed & \multicolumn{2}{c}{Camera} & \multicolumn{2}{c}{Average} & \multicolumn{2}{c}{Forget R.} \\
 & Model & MF1 & Acc & MF1 & Acc & MF1 & Acc & MF1 & Acc & MF1 & MF1 & Acc & MF1 & Acc & MF1 & Acc \\
\specialrule{.1em}{.05em}{.05em}
\multirow{4}{*}{Non-CL} & RoBERTa & 79.81 & 87.00 & 66.11 & 71.26 & 60.98 & 71.85 & 83.75 & 86.08 & 72.38 & 78.82 & 87.03 & 73.64 & 79.27 & \multicolumn{2}{c}{---} \\
 & RoBERTaDAP & 80.84 & \textbf{87.68} & 68.75 & 73.44 & 68.97 & 75.95 & 82.59 & 85.50 & 72.84 & 84.39 & 89.90 & 76.40 & 80.89 & \multicolumn{2}{c}{---} \\
 & AdapterDAP & 80.19 & 87.14 & 68.87 & 72.92 & 60.55 & 71.38 & 82.71 & 85.35 & 71.68 & 83.62 & 89.23 & 74.60 & 79.62 & \multicolumn{2}{c}{---} \\
 & PromptDAP & 79.00 & 86.45 & 66.66 & 71.35 & 61.47 & 72.36 & 84.17 & 86.53 & \textbf{73.09} & 85.52 & 90.38 & 74.98 & 80.03 & \multicolumn{2}{c}{---} \\
%  & CDS & 81.83 & 88.20 & 71.01 & 74.73 & 71.99 & 78.06 & 85.47 & 87.45 & 73.65 & 88.52 & 92.49 & 78.74 & 82.43 & \multicolumn{2}{c}{---} \\
\specialrule{.1em}{.05em}{.05em}
\multirow{11}{*}{CL} & NCL & 79.52 & 86.54 & 68.39 & 72.87 & 67.94 & 75.71 & 84.10 & 86.33 & 72.49 & 85.71 & 90.70 & 76.36 & 80.77 & 1.14 & 1.05 \\
 & AdapterCL & 80.13 & 87.05 & 67.39 & 72.30 & 57.71 & 69.87 & 83.32 & 85.86 & 72.07 & 83.70 & 89.71 & 74.05 & 79.48 & 0.15 & -0.02 \\
  & AdapterDEMIX & 79.99 & 87.12 & 68.46 & 72.73 & 63.35 & 72.86 & 78.07 & 82.42 & 71.73 & 86.59 & 91.12 & 74.70 & 79.66 & 0.74 & 0.36 \\
 & AdapterHAT & 79.29 & 86.70 & 68.25 & 72.87 & 64.84 & 73.67 & 81.44 & 84.56 & 71.61 & 82.37 & 89.27 & 74.63 & 79.78 & -0.23 & -0.18 \\
 & AdapterBCL & 78.97 & 86.52 & \textbf{70.71} & \textbf{74.58} & 66.26 & 74.55 & 81.70 & 84.63 & 71.99 & 85.06 & 90.51 & 75.78 & 80.46 & -0.06 & -0.19 \\
& AdapterCLASSIC & 79.89 & 87.05 & 67.30 & 72.11 & 59.84 & 71.08 & 84.02 & 86.22 & 69.83 & 86.93 & 91.25 & 74.63 & 79.59 & 0.44 & 0.25 \\
 & KD & 78.05 & 85.59 & 69.17 & 73.73 & 67.49 & 75.09 & 82.12 & 84.99 & 72.28 & 81.91 & 88.69 & 75.17 & 80.06 & -0.07 & 0.01 \\
 & EWC & \textbf{80.98} & 87.64 & 65.94 & 71.17 & 65.04 & 73.58 & 82.32 & 85.13 & 71.43 & 83.35 & 89.14 & 74.84 & 79.68 & 0.02 & -0.01 \\
& DER++ & 79.00 & 86.46 & 67.20 & 72.16 & 63.96 & 73.54 & 83.22 & 85.61 & 72.58 & 87.10 & 91.47 & 75.51 & 80.30 & 2.36 & 1.53 \\
 & HAT & 76.42 & 85.16 & 60.70 & 68.79 & 47.37 & 65.69 & 72.33 & 79.13 & 69.97 & 74.04 & 85.14 & 66.80 & 75.65 & -0.13 & -0.29 \\
  & HAT* & 74.94 & 83.93 & 52.08 & 63.94 & 34.16 & 56.07 & 64.71 & 74.43 & 68.14 & 65.54 & 81.44 & 59.93 & 71.33 & 3.23 & 1.83 \\
 & CDS & 80.34 & 87.16 & 69.36 & 74.01 & \textbf{70.93} & \textbf{77.46} & \textbf{85.99} & \textbf{87.70} & 72.80 & \textbf{88.16} & \textbf{92.30} & \textbf{77.93} & \textbf{81.91} & \textbf{-1.09} & \textbf{-0.60} \\
\specialrule{.1em}{.05em}{.05em}
\specialrule{.1em}{.05em}{.05em}
\end{tabular}}
\caption{End-task macro-F1 (MF1), accuracy and forgetting rate results 
% (Sec.~\ref{sec:results}) 
for all domains \textit{after continual DAP-training of all domains}, except for CHEMPORT in the PubMed domain, for which we use micro-F1 following~\cite{DBLP:conf/acl/GururanganMSLBD20,dery2021should,beltagy-etal-2019-scibert}. The results are averages of 5 random seeds (the domain training order is as they appear in the first row). Due to space limits, the results for \textit{different domain orders} and the \textit{standard deviations} are reported in Appendix~\ref{ap:order} and Appendix~\ref{ap:std}, respectively). Non-CL baselines has no forgetting. 
% \zixuan{Do we want to add TAPT results--- we are not better than MultiTask (MLM+CE) setting. Camera domain  checked}
} 
\label{tab:dapt_result}
\end{table*}




\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{cc|ccccccccccccccc}
\specialrule{.2em}{.1em}{.1em}
\multirow{2}{*}{Category} & Domain & \multicolumn{2}{c}{Restaurant} & \multicolumn{2}{c}{ACL} & \multicolumn{2}{c}{AI} & \multicolumn{2}{c}{Phone} & PubMed & \multicolumn{2}{c}{Camera} & \multicolumn{2}{c}{Average} & \multicolumn{2}{c}{Forget R.} \\
 & Model & MF1 & Acc & MF1 & Acc & MF1 & Acc & MF1 & Acc & MF1 & MF1 & Acc & MF1 & Acc & MF1 & Acc \\
\specialrule{.1em}{.05em}{.05em}
\multirow{5}{*}{Non-CL} & RoBERTa & 79.81 & 87.00 & 66.11 & 71.26 & 60.98 & 71.85 & 83.75 & 86.08 & 72.38 & 78.82 & 87.03 & 73.64 & 79.27 & \multicolumn{2}{c}{---} \\
 & RoBERTaDAP & 80.84 & \textbf{87.68} & 68.75 & 73.44 & 68.97 & 75.95 & 82.59 & 85.50 & 72.84 & 84.39 & 89.90 & 76.40 & 80.89 & \multicolumn{2}{c}{---} \\
 & AdapterDAP & 80.19 & 87.14 & 68.87 & 72.92 & 60.55 & 71.38 & 82.71 & 85.35 & 71.68 & 83.62 & 89.23 & 74.60 & 79.62 & \multicolumn{2}{c}{---} \\
 & PromptDAP & 79.00 & 86.45 & 66.66 & 71.35 & 61.47 & 72.36 & 84.17 & 86.53 & \textbf{73.09} & 85.52 & 90.38 & 74.98 & 80.03 & \multicolumn{2}{c}{---} \\
\specialrule{.1em}{.05em}{.05em}
%  & OURS (random) & 80.06 & 86.93 & 68.59 & 73.30 & 69.70 & 76.80 & 85.11 & 87.16 & 72.54 & 85.74 & 90.99 & 76.96 & 81.29 & -0.02 & 0.11 \\
\multirow{3}{*}{CL}  & CDS (-contrast) & \textbf{81.06} & 87.55 & 70.39 & 74.39 & 67.60 & 75.32 & 83.53 & 86.00 & 72.01 & 84.48 & 90.06 & 76.51 & 80.89 & -0.54 & -0.23 \\
 & CDS (-softmask) & 80.48 & 87.27 & 69.92 & 74.39 & 67.73 & 75.78 & 84.00 & 86.37 & 73.03 & 87.96 & 92.08 & 77.19 & 81.48 & -0.24 & -0.12 \\
 & CDS (-initialization) & 81.30  & 87.79 & 68.35 & 73.1 & 67.82 & 75.73 & 85.13 & 86.98 & 71.82 & 87.25 & 91.57 & 76.95 & 81.16 & 0.70 & 0.48 \\
 & CDS & 80.34 & 87.16 & \textbf{69.36} & \textbf{74.01} & \textbf{70.93} & \textbf{77.46} & \textbf{85.99} & \textbf{87.70} & 72.80 & \textbf{88.16} & \textbf{92.30} & \textbf{77.93} & \textbf{81.91} & \textbf{-1.09} & \textbf{-0.60} \\
\specialrule{.1em}{.05em}{.05em}
\specialrule{.1em}{.05em}{.05em}
\end{tabular}}
\vspace{-1mm}
\caption{Ablation results - averages of 5 random seeds. The \textit{standard deviations} are reported in Appendix~\ref{ap:std}. % \zixuan{you can read appendix as well}
% \zixuan{Appendix need update}
} 
\vspace{-4mm}
\label{tab:ablation}
\end{table*}


\vspace{-1mm}
\subsection{Results Analysis and Ablation Study}
\label{sec:results}
% \zixuan{need update}

{\color{black}Due to space limits, \textit{\textbf{Implementation Details}} are given in  Appendix~\ref{ap:imp_detail}}. Table~\ref{tab:dapt_result} reports the end-task results of all systems on the 6 datasets. The forgetting rate (\textbf{forget R.}) \cite{DBLP:conf/cvpr/LiuSLSS20} is computed as, $\frac{1}{t-1}\sum_{i=1}^{t-1}A_{i,i} - A_{t,i}$, where $A_{i,i}$ is the end-task performance right after its domain $i$ is DAP-trained, and $A_{t,i}$ is the performance of the end-task of domain $i$ after DAP-training the last domain. We average over all end-tasks except the last one as the last domain has no forgetting. The higher the forgetting rate is, the more forgetting it has. Negative rates indicate positive knowledge transfer. 
% \zixuan{We probably should separate the "average" and "individual datasets" in the results analysis --- I made changes in the following paragraphs}

%\textbf{Superiority of CDS.} 
Table~\ref{tab:dapt_result} shows that on average CDS outperforms all baselines and also achieve the best knowledge transfer. %Similar observations can be observed for individual domains except Restaurant, ACL and PubMed), CDS is almost the same as the best baseline. 
We discuss more observations bellow. % \bing{The observations below are out dated. I did not read.}

(1). RoBERTaDAP (traditional DAP-training) outperforms RoBERTa (non-DAP-training) on all datasets shows the benefit of DAP-training. % and indicates that MLM based DAP-training is a strong baseline. 

(2). Adapter (AdapterDAP) and prompt (PromptDAP) are similar on average, but poorer than CDS. This is because adapter and prompt both do not have sufficient trainable parameters, which are also randomly initialized and can be difficult to train. 

(3). RoBERTaDAP and NCL perform similarly. This shows RoBERTa is a strong model. NCL does not suffer much from catastrophic forgetting (CF). % CF is not a major problem. %, although NCL has some CF (see its forgetting rates).

(4). KD, EWC, DER++ and HAT are all poorer than NCL as they sacrifice learning performance to avoid CF. HAT performs poorly, indicating that \textbf{\textit{parameter-isolation}} is unsuitable for DAP-training as discussed in Sec.~\ref{sec:intro}. {\color{black}HAT* is even poorer as the features used in DAP-training (features from a sub-network in LM) are different from features used in end-task fine-tuning (features from the whole LM).} The adapter-based CL baselines (those with prefix ``Adapter'') cannot outperform non-CL AdapterDAP because they only focus on avoiding CF. AdapterDEMIX has some transfer but very weak. One exception is AdapterBCL, which can avoid CF while also achieving some transfer, but it is weaker than NCL. In general, CL baselines are all poorer than CDS as they don’t have methods to encourage knowledge transfer or they have to rely on adapters. %  and cannot directly work on Transformer \zixuan{remove "cannot directly work on Transforme" becuase we added the HAT baseline}. 
% \zixuan{one more reason is that they need to learn additional module}

\textbf{Knowledge transfer and forgetting avoidance.} 
% We now look at knowledge transfer and forgetting avoidance of CDS. 
{\color{black}Comparing the forgetting rates, we can see how the models {\color{black}fare} on CF and knowledge transfer.} CDS has the strongest negative forgetting rate, indicating it does well on both forgetting prevention and knowledge transfer. NCL, AdapterCL, AdapterDEMIX, EWC, KD and DER++ all suffer from some forgetting. HAT has no forgetting but it cannot {\color{black}learn well.} AdapterHAT and AdapterBCL have no forgetting but are weak in knowledge transfer.
% (3) MLM+AdaptedDeiT outperforms MLM+KD on 5 out of 6 datasets (except for Restaurant), while both of them are significantly poorer than CDS. This is because MLM+KD, though can see both general and specialized knowledge, struggles to find a good trade-off between them. Even though MLM+AdaptedDeiT may leverage the self-attention to combine the two knowledge, there is still no explicit control. What's worse, knowledge can be lost during  distillation.

% (4). Comparing the two contrastive learning baselines (MLM+SimCSE and MLM+TaCL), we see MLM+SimCSE is better than MLM+TaCL on 5 out of 6 datasets (except for Restaurant), while both are worse than CDS. This indicates that contrastive learning alone is insufficient, integrating the general and specialized knowledge is important for improving DAP-training. 
% \textbf{Effect of Forgetting Prevention.}
% \zixuan{If we want to show the effectiveness of our method in preventing forgetting, do we need to evaluate our model in the original general-purpose end-task?}
% \textbf{Effect of Contrastive Learning}

\textbf{Ablation.} % We are interested in knowing where the gain of CDS is from. 
% This leads to two questions: (1) is the soft mask helpful to DAPT? and (2) is the contrastive learning helpful to DAPT?. 
We conduct the following ablation experiments: \textbf{CDS (-contrast)} means that we remove the contrastive loss and only soft-mask the backward pass according to the importance. \textbf{CDS (-softmask)} means that we remove soft masking, and only use contrastive learning based on inputting the same input twice in Eq.~\ref{eq:contrast} {\color{black}(with the second term in the denominator removed)}. 
{\color{black}Table~\ref{tab:ablation} shows that the full CDS gives the best result on average and individual domains, except PubMed where CDS is very closed to CDS (-softmask),} indicating that every component contributes. 

% \textbf{CDS (random masking)} means that we randomly generate attention head importance and use them to soft-mask the attention heads. The contrastive loss is computed based on the ``general'' knowledge obtained with the random masks and the ``specialized'' knowledge obtained by not considering the masks when combining the attention heads. \textbf{Ensemble (LM+MLM)} performs the end-task fine-tuning on the MLM DAP-trained RoBERTa (conventional DAP-training) and the original RoBERTa (LM) by concatenating their outputs and take the average.
% \footnote{We don't have CDS(-soft-masking) because our contrastive learning relies on soft-masking. If removed, contrastive loss will not have the additional negative samples and our CDS becomes MLM+SimCSE.}


% Additional observations are as follows:

% (1) CDS (-softmask) outperforms RoBERTaDAP in average and most of the individual domains (two exceptions Restaurant and AI are almost the same), indicating that part of the performance gain is from the contrastive loss. 

% By comparing CDS (random mask) and CDS, we can see  CDS (random mask) is worse for all datasets, again indicating the soft masks are helpful.

% (2) CDS outperforms CDS (-contrast) on all datasets, indicating that another part of the gain is from soft masking because CDS only has two components (contrastive loss and soft masking). Though CDS (-contrast) is similar to RoBERTaDAP, the combination of soft masking and contrastive loss can further improve the performance. 


% \zixuan{I am a bit concerned because CDS(-contrast) is not much better than RoBERTaDAP and CDS (-softmask) is closed to CDS}

% This is confirmed by the fact that CDS (-softmask) outperforms RoBERTaDAP or is almost the same (Restaurant and AI).

% (3) Ensemble, which can see both the original LM and the traditional DAP-trained model during end-task fine-tuning, is weaker than CDS (-contrast) on 5 out of 6 datasets (except for Phone). This again indicates our soft masks are highly effective.

==> deprecated/sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}


\zixuan{make clear the difference between pre-training and post-training}

Pre-trained language models (LMs) like BERT~\citep{DBLP:conf/naacl/DevlinCLT19} and RoBERTa~\citep{DBLP:journals/corr/abs-1907-11692} %and GPT-3~\citep{brown2020language} 
significantly advanced NLP recently. A common way of applying an LM is to fine-tune it using the end-task data. % have become a standard component in almost all NLP applications. Representations learned by such LMs  achieve strong performances on many tasks. 
%with datasets of varying sizes and varying sources. 
%However, researchers found that large LMs are not universally effective: it is still helpful to build separate pre-trained models for specific domains~\citep{DBLP:conf/acl/GururanganMSLBD20,DBLP:conf/naacl/XuLSY19,xu2019review,sun2019fine,lee2020biobert,alsentzer2019publicly}. 
However, researchers have shown that using a large unlabeled domain corpus to further train an LM using the same training loss (e.g., the \textit{masked language model} (MLM) loss) to adapt the LM to the domain can help end-tasks in the domain to do even better~\citep{DBLP:conf/acl/GururanganMSLBD20,DBLP:conf/naacl/XuLSY19}. This further training of an LM is called \textit{post-training} or \textit{domain-adaptive pre-training}. % post-training uses a \textit{unlabeled} corpus in a specific domain to specialize or adapt the LM for the domain to improve the performance of end-tasks in the domain. It is typically applied \textit{before} \textit{supervised end-task fine-tuning}. A post-trained (post-trained) LM can be used by any end-task in the domain. The reason that unlabeled domain data helps is because post-training can effectively alleviate the domain-discrepancy between the pre-trained LM and end-tasks. 
\zixuan{The whole paragraph is about post-training, not related to what we really gooing to do}

This paper studies continual learning (CL) of post-training or \textit{continual post-training} to incrementally post-train a sequence of domain corpora $D_1, D_2, ...$. Once a domain is trained, its data is no longer accessible. In CL, each $D_i$ is called a \textit{task}, but we use the term \textit{domain} 
% in this paper 
to be consistent with post-training. 
% At any time, the post-trained LM can be used by any end-task in the trained domains. 
Continual post-training is important as in the real world, % the distribution of 
data shifts constantly and new domains keep emerging  \citep{DBLP:conf/acl/GururanganMSLBD20}.
% and the evolving nature of language itself over time \cite{???}. 
For example, one may adapt an LM trained over a general domain (e.g., News) to some science domains (e.g., ACL and AI papers). %~\citep{DBLP:conf/acl/LoWNKW20}). %and the distribution of incoming domain data may vary too. 
This requires LMs to continually learn new domains. {\color{black}This problem has some similarity to \textit{task-incremental learning} (TIL) of CL {\color{black}where the task id (domain id in our case) is needed in both training and testing}. However, we do not need domain ids in testing (i.e., end-task fine-tuning) to identify the right model to use.}
% \zixuan{define what is TIL?} 
% \zixuan{parameter? I feel model makes people think we are training separate model for different task. The same for the TST paper} to use. \zixuan{this sentence makes it sound like CPS also need the ID, because it says the problem setting needs ID by itself. I understand later we say CPS can address this but it is weird to say a problem need ID but we propose a model for the problem without ID needed}

Ideally, the proposed method should  have the following properties: \textbf{(1)} Maximally preserve the general language knowledge in the original LM. This is important because if it is forgotten in continual post-training, the knowledge learned from each domain alone will not be sufficient for good end-task performances. {\color{blue}Note that the general (language) knowledge is \textit{not all} knowledge in the LM. The LM should be able to be adapted to suit individual domains while preserving the general language knowledge.} \textbf{(2)} Overcome \textit{catastrophic forgetting} (CF),\footnote{\textit{Catastrophic forgetting}~\citep{McCloskey1989} in CL means that {\color{blue}the training of a new domain 
% needs to update the existing network, which 
may cause the performance degradation of the domains trained previously.}}  
% so that after post-training on a new domain, the knowledge learned for previous domains is not forgotten. 
{\color{blue} which is the same goal as conventional CL, i.e., we want to preserve \textit{all} knowledge in each individual domain/task.}
% \zixuan{(1) anbd (2) seem indeed both about forgetting. I think we can consider merge them up.}
\textbf{(3)} Encourage knowledge transfer across domains to achieve improved end-task performances % by leveraging the shared knowledge among domains 
compared to post-training each domain separately. {\color{black}\textbf{(4)} Need domain id for each end-task fine-tuning.} \zixuan{"need not"}
% \zixuan{should not?}% Note that domain id is needed for existing TIL systems. 

% \vspace{-1mm}
% TIL typically trains a sub-network for each task/domain in a shared network. 
A highly effective family of approaches for TIL is \textit{parameter-isolation} 
% \zixuan{This acronyms is probably not needed} (PI)
~\citep{Serra2018overcoming,wortsman2020supermasks}, which has almost no CF.
% \zixuan{some people thinks performance degradation means forgetting? regardless of reasons?}
It learns 
\textit{binary/hard masks} to isolate a sub-network for each task/domain. %In testing, the domain id is needed to use the right sub-network. 
However, this family is not suitable for continual post-training of an LM. The key issue is that this family is designed for supervised end-task CL. For CL post-training, we cannot isolate a sub-network for each domain simply because it means that end-tasks will not be able to use the general knowledge in the original LM, which results in very poor end-task performances (Sec.~\ref{sec:experiments}). % \zixuan{Will HAT, but use the whole LM to do fine-tuning (instead of the corresponding sub-network) also one of our baselines? But this may make things more complex}


This paper proposes a novel method, called CPS (\textit{C}ontinual \textit{P}ost-training of LMs with \textit{S}oft-masking), that has all 4 desired properties.~Instead of employing hard/binary masks, we propose \textit{soft-masks} that do not isolate a sub-network for each domain and as a result, the knowledge in the full model can be leveraged for end-task fine-tuning. % The proposed method is called CPS (\textit{C}ontinual \textit{P}ost-training of LMs with \textit{S}oft-masking). 
CPS directly updates the LM by exploiting over-parameterization of LMs as a large number of parameters in an LM are unimportant and can be pruned~\citep{li2021differentiable,michel2019sixteen}.  
In learning a new domain based on its unlabeled corpus, CPS overcomes CF by computing the importance of attention heads and neurons in Transformer layers for previous domains and soft-mask them based on their importance values to control the backward gradient flow to protect the previous domains knowledge  
(for simplicity, we use the term \textit{units} to mean both \textit{attention heads} and \textit{neurons} below).
However, this method cannot be applied to preserve the general knowledge in the original LM as we cannot directly find their important units (see Sec.~\ref{sec.initialization}). A novel proxy is proposed. In the forward pass, soft-masking is not applied, which encourages knowledge transfer across domains. {\color{black}CPS also contrasts the past domain (including both the general knowledge in the pre-trained LM and previous domain knowledge) representations and the full knowledge (including both the past domains and the current domain knowledge) to learn an integrated representation (Sec. \ref{sec:training}).\footnote{Contrasting the past domain and only the domain-specific knowledge gives poorer results (see Sec.~\ref{sec:results}) as it causes the two types of knowledge to split rather than to integrate.} } In end-task fine-tuning, unlike existing TIL methods, CPS does not need the domain id as the end-task data can automatically choose the right knowledge % in the resulting LM 
to use. % \zixuan{I feel it is because the forward pass does not masked so the feature learned from domain-specific data is consistent with the end-task. No evidence shows it can automatically choose --- if it can automatically chose the HAT but fine-tune with whole LM may also work}. 
Note that soft-masking has some resemblance to the regularization approach to CL, but it is quite different, which we detail in Sec.~\ref{sec:related}.  


% \zixuan{"in the following sections discussing the importance computation"}.

% This has two key advantages: 1) each domain still can exploit the general knowledge in the original LM. This is important and shared knowledge can be transferred across domains to achieve better end-task performances than existing post-training of each domain separately. 

\zixuan{in terms of CL post-training, I think we can claim we are the first one}
{\color{black}In summary, this} work makes the following contributions. 
\textbf{(i)} It discovers that the popular \textit{parameter-isolation} approach to TIL is unsuitable for continual post-training. % \zixuan{Is HAT also counts as PI? HAT is not as bad as HAT.}
%An entirely different method is needed. 
\textbf{(ii)} It proposes a novel soft-masking method to overcome CF and to encourage knowledge transfer. It further proposes to integrate knowledge across domains. To our knowledge, none of these has been done before. CPS also learns within an LM with no added structures or need for replay data. 
\textbf{(iii)} To preserve the general knowledge in the  LM, a novel proxy is proposed. Again, it has not been used before. \textbf{(iv)} Experiments have been conducted to demonstrate the effectiveness of CPS. Due to its ability to overcome CF and to transfer knowledge, we believe CPS has a great potential for practical applications.  

% \zixuan{reviewer has some different opinion to our argument}

% \zixuan{also talk about theoretically grounding, consider we are doing empirical research}

% CPS works by computing the importance of units in Transformer {\color{black}by partially borrowing some ideas from network pruning} and soft-masking them to deal with CF and to encourage knowledge transfer.  
% {\color{black}To our knowledge, this method is new.} CPS also learns directly within the MLM with no added structures and needs no replay data. 

% \input{sections/related}


==> deprecated/sections/proposal.tex <==

\section{Proposed CDS Technique}
\label{Sec: preliminary}


% \zixuan{the term “LM” need to be changed, once continual learning begins, there is no more LM. we probably need to explicitly differentiate LM, LM, MLM}


% \zixuan{added refer to figure,emphasized the contrasting between two type of knowledge}
% \ls{Paper needs more editing. The method part, we do not well break down the problem and explain how our solution address sub problems}

% CDS improves DAP-training by going beyond the MLM loss to  integrate the general knowledge in the LM and the specialized knowledge in the current domain. 

% \zixuan{main idea: 

% task 1: pre-trained general knoweldge; 

% task 2+: accumulate all mask

% Avoid forgetitng: constraint the trianing using importance-based soft mask;

% encourage transfer by contrastive, learning complemenetary knoweldge }

% \zixuan{Separate into 3 stages for each domain}


% \zixuan{all script will need a t. Or we omit the t script for simiplicity}


Continual DAP-training in CDS is based on two main ideas: (1) preserving the important previous knowledge by soft-masking units based on their importance to overcome CF, which also facilitates cross-task knowledge transfer. (2) encouraging the model to learn complementary representations of the current domain and previous domains {\color{black}(including the general knowledge in the LM, see below).}
Figure~\ref{fig:overview} gives an overview of CDS. 


\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\textwidth]{figure/ours.png}
 \vspace{-1mm}
\caption{
Illustration of CDS. 
% We omit the details of other parts in Transformer and only focus on the multi-head attention mechanism. 
(A) \textbf{Initialization} (Sec.~\ref{sec:initialization}) learns the importance of units (attention heads and neurons) for the general knowledge in LM. (B) \textbf{Training} (Sec.~\ref{sec:in_training}) trains the new domain using the importance scores as %the LM with the MLM loss and contrastive loss while 
soft-masks. % the parameters to preserve the previously learned domain knowledge. 
(C) {\color{black}\textbf{Importance Computation}} (Sec.~\ref{sec:after_training}) learns the importance of units for the current domain and combines with the importance accumulated over previous domains and the general knowledge. %. This is achieved by inserting a gate vector and computing the gradient-based importance. 
(D) illustrates the process of importance computation. The matrix represents the involved units in Transformer. Before training domain/task 1, we first learn the importance of units for the general knowledge in the LM. Since the importance scores are soft (rather than binary), we see all cells are colored with different shades of orange, indicating the difference in their importance scores (the number in each cell is the learned importance score). This importance score is used to constraining the training of domain/task 1 to preserve the important general knowledge in the LM. %and also used to compute a contrastive loss in \textbf{Training}. 
After training task 1, we first learn the important units for task 1 in \textbf{Importance Computation}. The different values in the green cells indicate the importance scores of units for task 1. We then combine (i.e., element-wise maximum) the importance with the accumulated importance for all previous domains (we can see mixed green and orange colors). % \zixuan{The values indicates accumulated importance}). 
The process is similar for task 2 and its importance scores are marked mostly in different shades of red.
% Attention heads are soft-masked based on attention heads importance $I'_{l,i}$ to preserve the important general knowledge in the LM. As an example, the first attention head is of importance score 0.9, indicating it is very important in the LM. We soft-mask its corresponding head by multiplying its gradient with 0.1 (see Eqs~\ref{eq:mask} and~\ref{eq.norm}), so we can see most part of the head becomes grey, indicating a strong soft-mask on the head. In contrast, the other two are less important (0.3) and thus most parts of the heads are still green, indicating that they are masked by a smaller soft-mask (0.7). 
% Some attention heads are soft-masked (the first and third attentions, in grey color) 
% The final objective of CDS consists of MLM on output with backward soft-masking applied and a contrastive loss which contrasts the output for \textit{general} knowledge ($\bm{o}^{\text{gen}}$ in Eq.~\ref{eq:general_knowledge}) and the output for \textit{specialized} knowledge ($\bm{o}^{\text{cur}}$ in Eq.~\ref{eq:specialized_knowledge})
% output with backward masking applied ($\bm{o}^{\text{specialized}}$
% with forward and backward soft-masking applied (the figure only shows backward soft-masking. We refer Eq.~\ref{general_knowledge} for  )
% \ls{forward/backward masking are unclear.}\zixuan{we probably no need to introduce the concept of ''forward masking''} \bing{I agree to get rid of forward pass}
% indicating the general knowledge) and output with backward masking applied ($\bm{o}^{\text{specialized}}$, indicating the current domain knowledge).
}
\label{fig:overview}
\vspace{-3mm}
\end{figure*}


% \subsection{Continual Learning and Pre-training}
% \zixuan{Do we need it?}
% \bing{I think we don't need to discuss continual learning here as we are doing continual learning.}


% \begin{algorithm}[]
% \DontPrintSemicolon
%   \KwInput{Dataset $D = (D^{(0)}, ..., D^{(T)})$}
%   \KwOutput{DAP-trained model, importance score for each domain $\{\bm{I}'\}$}
  
%   \SetKwProg{Fn}{Def}{:}{}
%   \Fn{\FInitialization{$D^{(t)}$,$\{\bm{I}\}$,$t$}}{
%         \If{$t = 0$} {$\bm{I}=\text{ProxyDistill}(D^{(t)})$ \label{alg:proxy}\Comment{See Eq.~\ref{eq:proxy}} \\}
        
%         \Else {$\bm{I}=\text{MaxPool}(\{\bm{I}\})$ \label{alg:maxpool} \Comment{See Eq.~\ref{eq:maxpool}} \\}
        
%         \KwRet $\bm{I}$\;
%   }
%   \;
%   \For{$t = 0,..,T $} 
%   { 
%      $\bm{I}=$\FInitialization$(D^{(t)},\{\bm{I}\},t)$ \\
%      \Comment{See Sec.~\ref{sec:initialization}} \\
     
%     \FTraining($D^{(t)},\bm{I})$ \label{alg:intraining}\\ \Comment{See Sec.~\ref{sec:in_training}} \\
    
%     $\bm{I}^{(t)}=$ \FPostProcess$(D^{(t)},t)$ \label{alg:afterttraining} \\
%     \Comment{See Sec.~\ref{sec:in_training}}\\ 
    
%     Append $I^{(t)}$ into the learned soft mask set $\{\bm{I}\}$. Store the $\{\bm{I}\}$. 
%   }
% \caption{Continual Learning in OURS}
% \label{algorithm_OURS}
% \end{algorithm}


To learn each new domain, two steps are involved. The first step is for \textbf{\textit{training}} (Sec.~\ref{sec:in_training}). It takes the importance scores of the units learned from previous domains and the new domain data as inputs to achieve (1) and (2). % on the new domain data while also preserving the previous knowledge by constraining the training using the importance scores as soft-masks. It also learns a good complementary representation for the new domain via contrasting the previous and the current domain knowledge . 
The second step is for \textbf{\textit{importance computation}} % \zixuan{Use a verb phrase as the name is a bit weird}
of units (Sec.~\ref{sec:after_training}). It learns the importance scores for the current domain and combines with the existing stored importance scores for previous domains. However, for the first domain/task, a different method (\textbf{\textit{initialization}}) is needed, {\color{black}which computes the importance of units to the general knowledge in the LM.} % the which we discuss next. \zixuan{we didn't explain why --- because we want to maintain and leverage the general knowledge. It would be not easy to find the importance units for general knowledge once CL begins.}

% To achieve (1) and (2), the training involves an  \FInitialization stage \textit{before} the starts of continual learning (Sec.~\ref{sec:initialization}). This stage prepares the parameter importance scores for \textit{general knowledge} in LM at different layers. 

% Figure~\ref{fig:overview} shows the overall framework of our proposed approach.

% It is worth noting that for the learning of the first domain, the importance of each parameter is computed based on the importance of the parameter to the \textit{general knowledge} in the LM. This happens in the \FInitialization stage for task/domain 1, not for the subsequent domains. For the rest domains, the parameter importance is computed in stage (3) by \FPostProcess.  
% because the LM is changed by the first domain and the generalized knowledge can be forgotten once the continual learning begins. 
% One key challenge is that the data used in training the LM is not accessible to users in practice. We propose an extra mechanism called \textit{proxy distillation} in Eq.~\ref{eq:proxy} to compute the importance without accessing to any of the LM's original training data. % ; After learning the importance score for general knowledge, our goal is to estimate the importance parameters for the \textit{domain-specific knowledge} (rather than general knowledge). This is achieved by learning in \FPostProcess with fully accessible to the current domain data.

% The above extra goal in task 1 causes difference between task 1 and subsequent tasks in \FInitialization, we will introduce both in detail. Algorithm~\ref{algorithm_OURS} shows the pseudo-code for our approach.



\subsection{Initialization: Computing units Importance for Task 1 Training}
\label{sec.initialization}
% \zixuan{do we want to mention "general knowledge" in 3.1 title? Why we need this initialization step is a bit vague now --- we only mention in the first sentence with "(general knowledge)"}
\label{sec:initialization}

% \FInitialization computes the importance of parameters to previous domains at different layers 
% \bing{this can be treated as initialization of CL as it is only applicable to the first task/domain. The writing would be cleaner that way. It is confusing currently. MaxPooling can be done in stage 3, right? Isn't it computed incrementally? Then we only need two stages. Section 3.1 will be initialization for Task/domain 1. Section 3.2 (InTraining) and 3.3 (AfterTraining computing the parameter importance) remain}.

This initialization step learns the importance of units (attention heads and neurons) in Transformer for the \textit{general} knowledge) before starting CL. The key components of a Transformer are \textit{multi-head attention layer}, \textit{intermediate layer} and \textit{output layer}. Below, we only discuss how to compute the importance scores of attention heads. The extension to neurons in the other layers is intuitive. To ease the notation, we omit task index $t$. The data used is only the new/current domain data.

\textbf{Multi-head attention.} %Multi-head attention is arguably the most important component in the Transformer model \cite{vaswani2017attention}. \zixuan{I feel the above sentence is unneccessay (we had this previously becaus in DGI we only soft mask attention head)} % We omit details of other parts and refer the reader to the original paper \cite{vaswani2017attention}. 
Let $\bm{x}=x^{(1)},...,x^{(b)}$ be a sequence of $B$ real vectors where $x^{(b)}\in\mathbb{R}^d$ and let $q\in\mathbb{R}^d$ be a query vector. 
% Figure~\ref{overview} (A) shows a conventional attention head.
The \textit{attention mechanism} is defined as 
\begin{equation}
\text{att}(\bm{x},q) = W_o\sum_{b=1}^B\alpha^{(b)}(q)W_vx^{(b)},
\end{equation}
where
\begin{equation}
\alpha^{(b)}(q)=\text{softmax}(\frac{q^TW_q^TW_kx^{(b)}}{\sqrt{d}}).
\end{equation}
The projection matrices $W_o, W_v, W_q, W_k\in\mathbb{R}^{d\times d}$ are learnable parameters. The query vector is from the same sequence as $\bm{x}$ in self-attention. A Transformer contains $L$ identical layers. For layer $l$, $n_l$ different attention heads are applied in parallel to enable the Transformer to be trained on more data. % Simply put, \textit{multi-head attention} (mhatt) is the simultaneous application of multiple attention heads in a single Transformer architecture. 
Multi-head attention (mhatt) is expressed as:\footnote{We follow the notation in \citep{michel2019sixteen}.} 
%where the notation in Eq.~\ref{eq:mhatt} is equivalent to the ``concatenation'' formulation in \cite{vaswani2017attention}.}%, in order to ease the exposition in the following sections.}.
\begin{equation}
\label{eq:mhatt}
\text{mhatt}_l(\bm{x},q)=\sum_{i=1}^{n_l}\text{att}_{l,i}(\bm{x},q),
\end{equation}
where $i$ indicates the $i^{th}$ attention head. Note, the input $\bm{x}$ is different for each layer since the input of a given layer is the output of the last layer. To ease the notation, we use $\bm{x}$ as input for all layers.

\textbf{Head importance.} Researchers have found that not all attention heads are important \cite{michel2019sixteen}. We introduce {\color{black}a \textit{gate vector}, where each cell is a \textit{gate variable}, $g_{l,i}$, for computing the importance of an attention heads.} % The resulting importance scores are used for soft-masking in DAP-training.
\begin{equation}
\label{eq:gmhatt}
\text{gmhatt}_l(\bm{x},q)=\sum_{i=1}^{n_l}g_{l,i} \odot\text{att}_{l,i}(\bm{x},q).
\end{equation}

A gradient-based head importance detection method is proposed in \cite{michel2019sixteen}. Given a dataset $D=\{(\bm{y}_m,\bm{x}_m)\}_{m=1}^M$ of $M$ samples  ($\bm{y}_m$ is the label of $\bm{x}_m$ as \cite{michel2019sixteen} worked on supervised learning), the importance of a head is estimated with a gradient-based proxy score
\begin{equation}
\label{eq:importance}
I_{l,i} = \frac{1}{M}\sum_{m=1}^M|\frac{\partial\mathcal{L}_{\text{importance}}(\bm{y}_m,\bm{x}_m)}{\partial g_{l,i}}|,
\end{equation}
where $\mathcal{L}_{\text{importance}}$ is a task-specific loss function. Note the gradient variable $g_{l,i}$ is initialized as all 1's, and is not changed. This is because we only care about the gradient and will not use the gradient to update the gate variable. In training (Sec.~\ref{sec:in_training} and Fig~\ref{fig:overview} (B)), the gate variable can be discarded. % \zixuan{added above sentence}% The gradient can be used as importance score because changing ${g_{l,i}}$ is liable to have a large effect on the model if $I_{l,i}$ has a high value. 
% \zixuan{we probably should use M instead of I to refer mask}

% Although Eq.~\ref{eq:importance} offers a way to compute the importance of attention heads \textit{w.r.t. a given loss $\mathcal{L}_{\text{importance}}$}, 
However, we are unable to directly apply Eq.~\ref{eq:importance} because class label is needed in Eq.~\ref{eq:importance} but our domain corpus is unlabeled in DAP-training. What is even more challenging is that we need to estimate the attention heads importance for the \textit{general knowledge} in LM but the data used in training the LM is not accessible to users of the LM.  %\bing{we may want to say that Eq.~\ref{eq:importance} needs class label information or supervised data} 
% domain-specific data is annotated and thus only have $(\bm{x}_m)$. 

To address these issues, we propose a \textit{proxy distillation loss} ($\mathcal{L}_{\text{proxy}}$) to replace $\mathcal{L}_{\text{importance}}$ to learn head importance for the general knowledge.


\textbf{Proxy distillation loss} 
% (line~\ref{alg:proxy} in Algorithm~\ref{algorithm_OURS}).
% We need a proxy for $\mathcal{L}_{\text{importance}}$ such that its gradient ($\nabla_{g_{l,i}}$) \footnote{For simplicity, we use $\nabla_{g_{l,i}}$ for the gradient in Eq.~\ref{eq:importance}.} can be used to compute head importance without using the LM's original pre-training data. 
We propose to use model \textit{robustness} as the proxy, i.e., we try to detect heads that are important for LM's \textit{robustness}. Its gradient, $\nabla_{g_{l,i}}$, then indicates the robustness and thus the importance to the LM model. Our rationale is as follows: If an $I_{l,i}$ has a high value, it indicates that it is important to the LM's robustness because its change can cause the LM to change a great deal. It is thus an important head. In contrast, if $I_{l,i}$ has a small value, it is a less or not important head.

To compute the \textit{robustness} of the LM, we take a subset of the current domain data $\{\bm{x}^{\text{sub}}_m\}$ (no label in DAP-training) and input $\bm{x}^{\text{sub}}_m$ twice to the LM and do distillation between the two resulting representations using KL-divergence,
\begin{equation}
\mathcal{L}_{\text{proxy}} = \text{KL}(f(\bm{x}^{\text{sub}}_m),f(\bm{x}^{\text{sub}}_m)),
\label{eq:proxy}
\end{equation}
where $f$ is the LM with different dropout masks. Note that we don't need to add any additional dropouts to implement $f$ because independently sampled \textit{dropout masks} are used as input in the Transformer. In training a Transformer, there are dropout masks placed on fully-connected layers and attention probabilities. Thus, simply feeding the same input to the Transformer twice will get two representations with different dropout masks. Since dropout is similar to adding noise, the difference between the two representations can be regarded as the \textit{robustness} of the Transformer model. 

 \vspace{-0.5mm}
\textbf{Extending to other layers.} For the other layers, we learn importance scores in a similar way. The only difference is that the importance is at attention heads level for multi-head attention layer but at the neurons level for intermediate and output layers.
Specifically, like that in Eq.~\ref{eq:gmhatt}, we first add a gate vector to the intermediate layer $\bm{g}^{\text{inter}}$ (consists of gate variables $g^{\text{inter}}_{l,i}$) 
% \zixuan{made the different between gate variable and gate vector more explicit} 
and a gate vector for the output layer $\bm{g}^{\text{output}}$ (consists of gate variables $g^{\text{output}}_{l,i}$) with the same size as the corresponding layer. We then use gradient-based detection method in Eq.~\ref{eq:importance} to learn the importance score of each neuron.

\textbf{From unit importance to parameter importance.} $I_{l,i}$ indicates the importance of each unit (an attention head or neuron) in layer $l$. We need to pass it to parameters for the soft-mask mechanism in the training step (Sec.~\ref{sec:in_training}). {\color{black}This is achieved  by simply applying the same importance $I_{l,i}$ to all the parameters (connections) leading to the unit.} % same size as the parameters, so that the parameters corresponding to the units can be soft-masked. \bing{not clear}} \zixuan{added "so that..."}
% \zixuan{why it is not understandable? expansion means copy to match the dimension}
% \begin{equation}
% \label{eq:importance_parameter}
% I_{l,i} = \text{expand}(I_{l,i},W_{l,i})
% \end{equation}


\subsection{Training: Learning New Domain, Soft-masking and Contrastive Loss}
\label{sec:in_training}


\textbf{Soft-masking units.}
% \zixuan{here should be parameters, we use the importance of attetion heads and neurons to soft-masks the parameters by expanding the importance and eq.8}
% (\FTraining, line~\ref{alg:intraining} in Algorithm~\ref{algorithm_OURS}). 
Recall we want to preserve the learned knowledge in the LM during DAP-training using the accumulated importance $I_{l,i}$ (including the importance for the general knowledge and learned domain-specific knowledge (see Sec.~\ref{sec:after_training}). As in Sec.~\ref{sec:initialization}, we only discuss soft-masking the multi-head attention layer. Other layers use the same mechanism. % \zixuan{added above sentence} 
Given the attention head $\text{att}(\bm{x},q)$ and the DAP-training loss $\mathcal{L}_{\text{DAP-train}}$ (typically the MLM loss; we also propose an additional loss in Eq.~\ref{eq:contrast}), we can ``soft mask'' its corresponding gradient ($\nabla_{\text{att}_{l,i}}$)~\footnote{$\nabla_{\text{att}_{l,i}}$ is the gradient for attention head $\text{att}_{l,i}(\bm{x},q)$, different from $\nabla_{g_{l,i}}$ in Eq.~\ref{eq:importance}, the gradient for gate variable $g_{l,i}$} using the head importance value $I_{l,i}$.
% \bing{What about other layers?}\zixuan{It is exact same as the the head by doing (1-importance)*gradient}
\begin{equation}
\label{eq:mask}
\nabla'_{\text{att}_{l,i}} = (1-I^{\text{norm}}_{l,i}) \odot \nabla_{\text{att}_{l,i}},
% \frac{\partial\mathcal{L}_{\text{DAP-training}}}{\partial \text{att}_{h}(\bm{x},q)}
\end{equation}
% \zixuan{Note in backward we use $(1-I)$, but in forward (next section) we use $I$. Do we want to emphasis that or it is already clear?} \bing{it is reasonably clear}
where $I^{\text{norm}}_{l,i}$ is from $I_{l,i}$ via normalization
\begin{equation}
% \label{eq:gradient_mask}
I^{\text{norm}}_{l,i} = |\text{Tanh}(\text{Normalize}(I_{l,i}))|.
\label{eq.norm}
\end{equation}
Normalization makes the $I_{l,i}$ have a mean of 0 and standard deviation of 1. Absolute value of $\text{Tanh}$ ensures that $I_{l,i}$ takes values in the interval $[0,1]$.  Eq.~\ref{eq:mask} constrains the gradient of the corresponding head $\text{att}_{l,i}(\bm{x},q)$ by element-wise multiplying the gradient with one minus the head importance. As mentioned in Sec.~\ref{sec:initialization}, we expand ({\color{black}by copying}) the importance $I_{l,i}$ to match the dimensions of $\nabla_{\text{att}_{l,i}}$ {\color{black}to applying it to all associated parameters.} This is \textit{soft-masking} because $I_{l,i}$ is a real number in $[0,1]$ (instead of binary \{0, 1\}), which gives the model the flexibility to adjust any attention head. This is useful because although some heads are important, they may conflict with the knowledge in the current domain and thus need some small adjustments. % \zixuan{this makes it sound like forgetting is possible because it adjusts toward current domains. We may just want to say it makes transfer possible}% \zixuan{This is useful because knowledge transfer between learned domains and current domain becomes possible (comparing to hard mask which fixes all the learned knowledge).
% Note that the mask here only affects the backward pass and is not used in the forward pass. 
% In the next section, we will introduce how we use the masks in forward pass \zixuan{maybe just say "how to use the importance score", instead of saying "mask in forward", which could be confusing}to enable the general knowledge to help current domain DAP-training. \zixuan{still say "help"}
Figure~\ref{fig:overview} (D) shows the units are soft-masked (in different colors and values). % \bing{I do not see that}
% some attention heads (the first and third ones, in grey color) are soft-masked 
% \bing{The figure does not show different $\bm{I}_h$ values that soft-masks every head, }.

\vspace{+1mm}
\noindent\textbf{Contrasting the previously learned and new domain knowledge.}
% \label{sec.contrast}
% Sec.~\ref{sec: prevent_forgetting} discussed how to preserve the general knowledge. 
% \zixuan{need update: all "general" should change to "Learned" knowledge}
% We have seen how we soft-mask the learned units to preserve the learned knowledge. 
We now present how to integrate the previously learned knowledge and the current domain knowledge. We first introduce how we obtain the learned knowledge from the LM and the current domain for the input $\bm{x}$, and then discuss how we contrast them to achieve their integration. As in Sec.~\ref{sec:initialization}, we focus only on the attention head layer, and it is easy to extend to the other layers.% We do not contrast different input  \zixuan{we still have in-batch negative, risky to say do not contrast differnt input} or augmented samples.

\textbf{(1)} \textit{Obtaining previously learned knowledge in the current LM using the input $\bm{x}$}. % \bing{This part is confusing. I made a lot of changes. Check}\zixuan{Probably because we copied too many from previous submission about GLM and specialized knowledge}.
This is done by extracting the representation of $\bm{x}$ from the network of the previous domains by combining the attention heads and their importance scores ($I^{\text{norm}}_{l,i}$ in Eq.~\ref{eq.norm}) in a forward pass. Note that this is the accumulated importance for all previous domains {the general knowledge} (see Sec.~\ref{sec:after_training}). Formally, we plugin $I^{\text{norm}}_{l,i}$ as the gate variable $g_{l,i}$ in Eq.~\ref{eq:gmhatt},
\begin{equation}
\label{eq:general_knowledge}
\text{gmhatt}^{\text{prev}}_l(\bm{x},q)=\sum_{n=1}^{n_l}I^{\text{norm}}_{l,i} \odot\text{att}_{l,i}(\bm{x},q).
\end{equation}
Given the attention heads for the previously learned knowledge $\text{gmhatt}^{\text{prev}}_l$, we can plug it into the whole Transformer to obtain the final learned knowledge or representation (taking the average of each token's output in the input sequence $\bm{x}$).
\begin{equation}
\label{eq:final_general_knowledge}
\bm{o}^{\text{prev}} = \text{Transformer}(\text{gmhatt}^{\text{prev}}(\bm{x},q)).
\end{equation}
{\color{black}(See $\bm{o}^{\text{prev}}$ also in Figure~\ref{fig:overview} (B)).} %   shows the obtained general knowledge representation from applying backward soft-masking (Eq.~\ref{eq:mask}).} \zixuan{and plugin in importance as gate variable (Eqs~\ref{eq:general_knowledge} and \ref{eq:final_general_knowledge})?} % and conditioning on the head importance soft-masks (Eq.~\ref{eq:final_general_knowledge}). % \bing{deleting forward mask}\zixuan{deleted}

\textbf{(2)} \textit{Obtaining current domain knowledge in $\bm{x}$}. This is similar to the above. The only difference is that we extract the representation by combining all attention heads without considering their importance. % as when we learn the specialized knowledge for the new domain, the forward flow is not effected by the soft-masks\bing{why?}\zixuan{why it is hard to understand?}.
% \bing{why} \zixuan{because soft-mask only block the backward pass, so the current domain representation is simply the representation from not considering importance. we also emphasis this in previous sub-section}. 
Formally, we remove the gate when combining the attention heads,
\begin{equation}
\label{eq:specialized_knowledge}
\text{gmhatt}^{\text{cur}}_l(\bm{x},q)=\sum_{i=1}^{n_l}\text{att}_{l,i}(\bm{x},q).
\end{equation}
% to get the current domain knowledge $\text{gmhatt}_l(\bm{x},q)$ 
Similarly, we can plug it into the Transformer,
\begin{equation}
\label{eq:final_specialized_knowledge}
\bm{o}^{\text{cur}} = \text{Transformer}(\text{gmhatt}^{\text{cur}}(\bm{x},q)).
\end{equation}
(See $\bm{o}^{\text{cur}}$ also in Figure~\ref{fig:overview} (B)). 
% $\bm{o}^{\text{cur}}$ shows the obtained specialized domain knowledge {\color{red}from applying backward (Eq.~\ref{eq:mask}) mask\zixuan{soft-mask?} and removing gate variable (Eqs.~\zixuan{\ref{eq:specialized_knowledge} and}  \ref{eq:final_specialized_knowledge}).} %\zixuan{change the notation from v to o to consistent with the figure}

%\bing{give a bit more explanation}.

\textbf{(3)} \textit{Contrasting learned and current domain knowledge.}
% (line~\ref{alg:intraining} in Algorithm~\ref{algorithm_OURS}). 
Contrastive learning helps learn a good isotropic representation that is good for down-stream tasks, with the help of positive $\bm{o}_m^+$ and negative $\bm{o}_m^-$ instances.  In our case, such instances are representations of the input $\bm{x}$ in both the current domain and the previously learned domain knowledge in the current LM. %\bing{aren't they both from the current LM?}\zixuan{update the sentence}. 
This enables us to contrast the two representations, %and force them to be different, 
which essentially makes the two representations \textit{complementary} as they represent two aspects of the same input. It thus encourages the current domain representation of $\bm{x}$
% ($\bm{o}^{\text{cur}}$) 
to learn knowledge that is not already in the learned knowledge in previous domains. 
% represented by ($\bm{o}^{\text{prev}}$). % of the same input $\bm{x}$. % \bing{why complementary}. 
% \zixuan{no good reason yet}

We construct the contrastive instances as follows: for an input $\bm{x}_m$, three contrastive instances are produced. Anchor $\bm{o}_m$ and positive instance $\bm{o}_m^+$ are both the current domain specialized knowledge from  Eq.~\ref{eq:final_specialized_knowledge}, obtained based on two independently sampled dropout masks in Transformer (recall that this can be achieved by inputting $\bm{x}_m$ twice, see Sec.~\ref{sec:initialization}). $\bm{o}_m^+$ and $\bm{o}_m$ are positive instances as the dropout noise has been shown good positive instances for improving alignment in training sentence embedding~\cite{gao2021simcse}. Negative instance $\bm{o}_m^-$ is the representation of $\bm{x}_m$ in the previously learned knowledge obtained by Eq.~\ref{eq:final_general_knowledge}. 
Contrastive learning pushes the positive and negative instances away, forcing them to be different and covering different aspects (previously learned and domain specialized) of the same input, resulting in a complementary effect or knowledge integration.
% \zixuan{removed 'uniformity' and "discriminative"}.

{\color{black}Formally, with $\bm{o}_m$, $\bm{o}_m^+$, and $\bm{o}_m^-$, our contrastive loss is ($\text{sim}(\cdot)$ is the cosine similarity), % \bing{Eq (1) \& (14) very different? Triplet loss?}
\begin{equation}
\label{eq:contrast}
\small
\mathcal{L}_{\text{contrast}} =  -\text{log}\frac{e^{\text{sim}(\bm{o}_m,\bm{o}_m^+)}/\tau}{\sum_{j=1}^N(e^{\text{sim}(\bm{o}_m,\bm{o}_j^+)/\tau}+e^{\text{sim}(\bm{o}_m,\bm{o}_j^-)/\tau})}.
\end{equation}
%where $N$ is the mini-batch size, {\color{black}$\tau$ is a temperature unit}, \zixuan{we probably don't need to explain N and $\tau$ because they already explain in related work}and $\text{sim}(\cdot)$ is the cosine similarity. 
Compared to Eq.~\ref{eq.relate_contrast},
% \zixuan{here we compare the related work, probably the related work of contrastive loss is needed} 
the second term is added in the denominator, i.e., representation in the previously learned knowledge as additional negative instances. Figure~\ref{fig:overview} (B) shows a red arrow pointed from $\bm{o}^{\text{cur}}$ to itself, indicating the positive instances are from inputting twice. The dashed red arrow pointing to $\bm{o}^{\text{prev}}$ indicates the negative instances contrasting the specialized and previously learned knowledge.}


%  \zixuan{achieve complementary effect?}. \zixuan{+"Different from the existing contrastive learning which requires augmented samples, our contrastive learning contrasts between two views (specialized and general representations) for \textit{the same input}. We call this ``''". It forces the two views to be different and covering different aspects (general and specialized) for the same input. We call this \textit{complementary effects}} \zixuan{I feel the key for "complementary" to make sense is that they are different view for the same input}


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc|ccccc}
\specialrule{.2em}{.1em}{.1em}
\multicolumn{3}{c|}{Unlabelde Domain Datasets} & \multicolumn{5}{c}{End-Task Classification Datasets} \\
Source & Dataset & Size & Dataset & Task & \#Training & \#Testing & \#Classes \\
\specialrule{.1em}{.05em}{.05em}
\multirow{3}{*}{Reviews} & Yelp Restaurant & 758MB & Restaurant & Aspect Sentiment Classification (ASC) & 3,452 & 1,120 & 3 \\
 & Amazon Phone & 724MB & Phone & Aspect Sentiment Classification (ASC) &  239 & 553 & 2 \\
 & Amazon Camera & 319MB & Camera & Aspect Sentiment Classification (ASC) & 230 & 626 & 2 \\
 \hline
\multirow{3}{*}{Academic Papers} & ACL Papers & 867MB & ACL & Citation Intent Classification & 1,520 & 421 & 6 \\
 & AI Papers & 507MB & AI & Relation   Classification & 2,260 & 2,388 & 7 \\
 & PubMed Papers & 989MB & PubMed & Chemical-protein Interaction Prediction & 2,667 & 7,398 & 13 \\
\specialrule{.1em}{.05em}{.05em}
\end{tabular}
}
\caption{
% \zixuan{change to our dataset (MNLI and DBPdia are removed)} 
% \zixuan{It is weird to me why we add MNLI, it is not in the same domain as BANKING77/CLINIC. Without supervision, this seems to be meaningless? Any good to use a unrelated datasets?} 
Statistics of datasets for DAP-training. Their end-task supervised learning datasets are in Appendix~\ref{ap:dataset}.  % \zixuan{we may want to explain more about those task (mentioned by one reviewer) \bing{I agree}} 
} 
\label{tab:dataset}
\vspace{-4mm}
\end{table*}

\vspace{+1mm}
\noindent
\textbf{Final Loss Function}.
% CDS is a pipelined model: First, {\color{black}a subset of the domain data} is used to estimate the attention head importance ($I_{l,i}$ in Sec.~\ref{sec: prevent_forgetting}). Second,
The final DAP-training loss combines the Masked Language Model (MLM) loss after applying the proposed soft-masking for the general knowledge (we call $\mathcal{L}_{\text{MLM+}}$) (Sec.~\ref{sec:initialization}) and the proposed contrastive loss:
\begin{equation}
\label{eq:final_loss}
\mathcal{L}_{\text{DAP-train}} = \mathcal{L}_{\text{MLM+}} + \lambda_1\mathcal{L}_{\text{contrast}}
\end{equation}
where {\color{black}$\lambda_1$ is a hyper-parameter}. %to adjust the impact of the added term. \zixuan{why MLM+ subscript?}


\subsection{Compute Importance: Learning and Accumulating Importance for Future Use}
% (line~\ref{alg:afterttraining} in Algorithm~\ref{algorithm_OURS})}
\label{sec:after_training}

After training the new/current domain, we learn the units importance by applying Eq.~\ref{eq:importance} for the domain in a self-supervised manner. Similar to the computation of $\mathcal{L}_{\text{proxy}}$ in Eq.~\ref{eq:proxy}, we randomly sample a subset (a hyper-parameter) of the current domain data $\{(\bm{y}^{\text{sub}}_m,\bm{x}^{\text{sub}}_m)\}$, where $\bm{x}^{\text{sub}}_m$ is the input and $\bm{y}^{\text{sub}}_m$ is the masked token as in MLM self-supervised loss. We can then easily compute the importance $I_{l,i}$ via $\mathcal{L}_{\text{MLM}}$ (we do not need $\mathcal{L}_{\text{proxy}}$ as we can directly use the current domain data).
% The resulting $\bm{I}$ is appended to the set $\{\bm{I}\}$ and stored for use in learning the next domain.


% \textbf{Accumulating all previous importance}
% (line~\ref{alg:maxpool} in Algorithm~\ref{algorithm_OURS}).
% Proxy distillation loss helps us learn the importance attention head for general knowledge in LM. 
% As shown in Algorithm~\ref{algorithm_OURS}, we store the learned importance all along the continual process.
% For subsequent tasks, we no longer need to do proxy distillation because the LM has changed toward domain-specific. 
The resulting $I_{l,i}$ is added to the accumulated importance of the previous domains, %so that we can know what heads are important for previous domains, 
via element-wise maximum {\color{black}(EMax)}, %\bing{what about subsequent tasks? Can the following be computed incrementally? Then there is no need to save the importance scores for each task, right?}
\begin{equation}
I^{(t)}_{l,i} = \text{EMax}(\{I_{l,i},I^{(i_{\text{prev}})}_{l,i}\}),
\label{eq:maxpool}
\end{equation}
where %$i_{\text{prev}}$ is the id of the previous domain and
$I^{(i_{\text{prev}})}_{l,i}$ refers to the previously accumulated importance. The resulting $I^{(t)}_{l,i}$ will be used for task $t+1$ (Sec.~\ref{sec:in_training}, where we omit the superscript $t$). 


==> deprecated/sections/related.tex <==

% \zixuan{May need continual learning related work, consider those in "\url{https://www.overleaf.com/8166731134zpndccxcmkyh}"}

% Our work is related to several topics. % We review their literature and compare them with our work. % \bing{I think that some content explaining different topics should go to the Introduction}

%\vspace{+1mm}
% \noindent
\textbf{Post-training} (also known as domain-adaptive pre-training).
Researchers have applied post-training to many domains, e.g., reviews \citep{DBLP:conf/naacl/XuLSY19,sun2019fine}, % biomedical text \citep{lee2020biobert,alsentzer2019publicly}, 
news and academic papers \citep{DBLP:conf/acl/GururanganMSLBD20}, % social media \citep{chakrabarty2019imho} 
and shown improved end-task results. % and court documents \citep{gururangan2021demix}. 
However, they are not about CL. 
% all use the same mask language model (MLM) loss and are not concerned with CL. % {\color{black}The MLM loss is insufficient. It is important to explicitly {preserve} important general knowledge in the LM and to make general and domain knowledge complementary.} % encourage it to help the current domain learning. \zixuan{this sentence says "help each other", also need change} 

% \vspace{+1mm}
\noindent
\textbf{Continual learning.} % \zixuan{Need more CL related work, consider those in "\url{https://www.overleaf.com/8166731134zpndccxcmkyh}"} % As we want to preserve important knowledge in the LM in post-training, our work is related to  \textit{catastrophic forgetting} (CF) prevention in \textit{continual learning} (CL). CL learns a sequence of tasks incrementally. CF means that in learning each new task, the system may change the parameters learned for previous tasks and cause their performance to degrade~\citep{mccloskey1989catastrophic}. In post-training, adapting the LM with the current domain data naturally causes forgetting of some knowledge in the LM. 
Many approaches have been proposed to overcome CF: 
(1) \textit{Regularization methods}~\citep{Kirkpatrick2017overcoming,Seff2017continual} computes the importance of each parameter to previous tasks and uses a regularization term to penalize the sum of changes.
%add a regularization to ensure minimal changes to important parameters for previous tasks. 
Our CPS is related to 
%the regularization method 
EWC~\citep{Kirkpatrick2017overcoming}, 
but they are different. % EWC computes the importance of each parameter to previous tasks and uses a regularization term in its loss function to penalize the sum of changes to the important parameters. 
(1) CPS does not control each parameter/weight, but only attention heads or neurons based on their importance scores. This gives less forgetting (see the forgetting rate in Table~\ref{tab:dapt_result}) because even a small change to each parameter for a neuron can give a large total change to the neuron's activation. (2) CPS directly controls the backward gradient flow on each neuron, which is more fine-grained and effective than the sum of changes of all parameters. Our experimental results confirms EWC is significantly poorer than CPS (see Table~\ref{tab:dapt_result}). (2) \textit{Replay methods} retain~\citep{Rebuffi2017,wang2020efficient} or generate some data of old tasks~\citep{Shin2017continual,He2018overcoming} and use them in learning a new task;
(3) \textit{parameter-isolation methods} \citep{Serra2018overcoming,wortsman2020supermasks} allocate neurons and parameters for different tasks and mask them in task learning. This family has almost no CF in \textit{task-incremental learning} setting where the domain id is known in any time. However, this family is designed for supervised end-task CL and learns \textit{binary/hard masks} to isolate a sub-network for each domain. For continual post-training, we cannot isolate a sub-network for each domain because it means that end-tasks cannot use the general knowledge in the LM, which results in very poor end-task performances.

% None of these approaches is for continual post-training, which needs a different method in the context of an LM as we elaborated in the introduction section. % Our approach is more related to parameter-isolation, but we do not use binary masks and o 

% Furthermore, since tasks in these applications are very similar, KT is fairly straightforward and there is little need to choose similar tasks for selective knowledge transfer, which is needed in CDL because different domains can be quite different. The proposed approach in CDL is also different.

